Compact Graph Architecture for Speech Emotion Recognition

We propose a deep graph approach to address the task of speech emotion recognition. A compact, efficient and scalable way to represent data is in the form of graphs. Following the theory of graph signal processing, we propose to model speech signal as a cycle graph or a line graph. Such graph structure enables us to construct a Graph Convolution Network (GCN)-based architecture that can perform an accurate graph convolution in contrast to the approximate convolution used in standard GCNs. We evaluated the performance of our model for speech emotion recognition on the popular IEMOCAP and MSP-IMPROV databases. Our model outperforms standard GCN and other relevant deep graph architectures indicating the effectiveness of our approach. When compared with existing speech emotion recognition methods, our model achieves comparable performance to the state-of-the-art with significantly fewer learnable parameters (~30K) indicating its applicability in resource-constrained devices.

==> tex/related.tex <==
In this section, we review the related work in the areas of GCNs and speech emotion recognition.

\noindent\textbf{Graph neural network.} Due to popularity and success of Convolution Neural Network (CNN), considerable research effort \cite{bruna2013spectral,xu2018how,kipf2017semi} has been done to design CNN for graph data. The GCNs has been classified into \textit{spatial} and \textit{spectral} which we focus on spectral method in this paper. Spectral-based methods have a solid foundation in graph signal processing \cite{6494675}. The first prominant research \cite{bruna2013spectral} on GCNs generalized convolution operation on the spectrum of the graph Laplacian and assumed convolution kernel matrix as a diagonal set of learnable parameters. In a follow-up work, ChebNet \cite{defferrard2016convolutional} was proposed to reduce computational cost by computing kernels recursively in terms of Chebyshev polynomials. Later in a recent work \cite{kipf2017semi}, a first order approximation of ChebNet was used to further simplify the convolution to a linear operation. Although recent works reduce the computation burden, they also lose information. In this paper, we follow the original definition of convolution in spectral graph domain.

\noindent\textbf{Speech emotion recognition.} Most works in the area of SER, follow a similar steps. First, preprocess the raw audio to extract low-level descriptors (LLDs) (due to difficulty of speech analysis compare to image) and then give them to deep networks to generate emotion labels \cite{tang2018end,zhao2018exploring,huang2016attention,mirsamadi2017automatic}. Extracting acoustic features is more common while pretrained \cite{zhang2019few} or lexical features \cite{jin2015speech} has been shown to be useful. Speech-based classification methods have been categorized into two main groups. First category treat the speech as a dynamic process where dynamical models such as Hidden Markov Models (HMM) \cite{schuller2003hidden} and Recurrent Neural Networks (RNN) \cite{huang2016attention,mirsamadi2017automatic}. The second category uses LLDs directly without considering any time dependency such as Support Vector Machine (SVM) \cite{wang2015speech,mangalam2017learning} and CNNs \cite{mao2019deep}.
